A Robust Asymmetric Kernel Function for Bayesian Optimization, with Application to Image Defect Detection in Manufacturing Systems

Some response surface functions in complex engineering systems are usually highly nonlinear, unformed, and expensive-to-evaluate. To tackle this challenge, Bayesian optimization, which conducts sequential design via a posterior distribution over the objective function, is a critical method used to find the global optimum of black-box functions. Kernel functions play an important role in shaping the posterior distribution of the estimated function. The widely used kernel function, e.g., radial basis function (RBF), is very vulnerable and susceptible to outliers; the existence of outliers is causing its Gaussian process surrogate model to be sporadic. In this paper, we propose a robust kernel function, Asymmetric Elastic Net Radial Basis Function (AEN-RBF). Its validity as a kernel function and computational complexity are evaluated. When compared to the baseline RBF kernel, we prove theoretically that AEN-RBF can realize smaller mean squared prediction error under mild conditions. The proposed AEN-RBF kernel function can also realize faster convergence to the global optimum. We also show that the AEN-RBF kernel function is less sensitive to outliers, and hence improves the robustness of the corresponding Bayesian optimization with Gaussian processes. Through extensive evaluations carried out on synthetic and real-world optimization problems, we show that AEN-RBF outperforms existing benchmark kernel functions.

==> tables/FFNN_parameters.tex <==
\begin{table}[!t]
\renewcommand{\arraystretch}{1.3}
\footnotesize
\centering
\caption{The parameters and hyperparameters of the feed-forward neural network (FFNN).}
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c|}
\hline
\textbf{Parameter}                         & \textbf{Value}  \\ \hline
Hidden layers of Conv2D 1                  & 32              \\ \hline
Hidden layers of Conv2D 2                  & 64              \\ \hline
Filter size of Conv2D 1 & Conv2D 2         & (3, 3)          \\ \hline
Activation function of Conv2D 1 & Conv2D 2 & ReLU            \\ \hline
Filter size of MaxPooling                  & (2, 2)          \\ \hline
Activation function of Dense               & Softmax         \\ \hline
Optimizer                                  & Adam            \\ \hline
\textbf{Hyperparameter}                    & \textbf{Domain} \\ \hline
Dropout rate                               & (0.25, 0.75)    \\ \hline
Learning rate of Adam optimizer            & (0.00001, 0.1)  \\ \hline
\end{tabular}}
\label{tab:FFNN_parameters}
\end{table}
